SketchEmbedNet: Learning Novel Concepts by Imitating Drawings

Sketch drawings capture the salient information of visual concepts. Previous work has shown that neural networks are capable of producing sketches of natural objects drawn from a small number of classes. While earlier approaches focus on generation quality or retrieval, we explore properties of image representations learned by training a model to produce sketches of images. We show that this generative, class-agnostic model produces informative embeddings of images from novel examples, classes, and even novel datasets in a few-shot setting. Additionally, we find that these learned representations exhibit interesting structure and compositionality.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/classification.tex <==
% !TEX root = ../main.tex
\input{sections/tables/tab_classification}
\input{sections/tables/tab_fsl_omniglot}
\section{Classification using \modelembedding{}s}
\label{sec:classification}
A major objective of representation learning is to produce salient and generalizable representations of the input space. We evaluate \modelembedding{}s by classifying examples of novel examples and classes from the training dataset \MR{revisit}. We also extend our evaluation to a stronger notion of generalization by classifying unseen datasets in a challenging few-shot classification task without any further adaptation or label supervision.

\model{} is trained as described in Section~\ref{sec:method}, one model instance for each dataset in~\ref{sec:training_data} after which the weights are frozen. Embeddings are extracted using the CNN encoder and are made deterministic by only taking the mean of the random normal latent space $z$. The variance parameter is discarded. Only a single model is trained on each dataset and is used throughout the entire section. No labels were observed during training \model{}. 

\subsection{Classifying novel examples and classes}
\label{sec:novel_classification}
We compare our \modelembedding{} method with other label-free representation learning approaches. We train a variational autoencoder (VAE)~\citep{vae} and a contrastive model using the InfoNCE loss~\citep{Oord2018infonce} which also uses sequential sketch supervision. An additional pix2pix~\citep{pix2pix} model is trained to map natural images and rendered sketches for the Sketchy dataset. Models trained on the Quickdraw dataset use the Conv4 architecture from~\citet{vinyals2016matching} while embedding images while Sketchy-trained models use the ResNet-12~\cite{oreshkin2018tadam} architecture. The InfoNCE model uses a RNN for encoding sketch inputs and individual and shared linear projection layers for the separate image and sketch encoding branches similar to the search embedding procedure in~\citet{sketchformer}.

\paragraph{Linear classification protocol.} A supervised linear classifier (fully-connected layer with softmax activations) is trained on embeddings extracted from a set of training examples. We report the classification accuracy on embeddings of a set of test examples. 

\paragraph{Quickdraw classification.} Training data consists of 256 labelled examples of each class. Novel example generalization is evaluated in 300-way classification on unseen examples of training classes; novel class generalization is evaluated on 45-way classification of unseen Quickdraw classes. Results presented in Table~\ref{tab:classification_quickdraw}.

\paragraph{Sketchy classification.} Due to the limited data in Sketchy, generalization is evaluated on the 1000-way classification ILSVRC2012 benchmark~\citep{ILSVRC15}. Results presented in Table~\ref{tab:classification_sketchy}.
\begin{figure}[t]
    \centering
    \includegraphics[trim=0.05cm 0.05cm 7cm 6.7cm,clip,width=0.48\textwidth]{figures/seen_samples.pdf}
    \caption{Sketches of seen examples}
    \label{fig:seen_samples}
\end{figure}

\subsection{Few-shot classification of unseen datasets.}
\input{sections/tables/tab_fsl_mii}
We extend the notion of generalization by evaluating on entirely unseen datasets. We evaluate our Quickdraw-trained model on the Omniglot dataset of handwritten characters~\citep{Lake2015bpl} and the Sketchy-trained model on the mini-ImageNet benchmark~\citep{vinyals2016matching}. Not only are are the classes different but the entire distribution of classes is different from the training data.

\paragraph{Few-shot experimental setup.} We formulate few-shot classification as an episodic, $N$-way, $K$-shot classification. At testing, a ``task'' is sampled consisting of a labelled ``support'' set of $K$ examples for each of $N$ randomly selected classes is used to train a linear classifier in the same way as in Section~\ref{sec:novel_classification}. The learned linear classifier is then evaluated on a ``query'' set of unseen examples from each of the $N$ classes and accuracy is reported. \AW{Fuse this into 1 sentence in the above paragraph}

\paragraph{Comparison to unsupervised few-shot classification.} In conventional few-shot classification, models are trained on labelled episodes consisting of classes from the same class and dataset distribution as those present during test time. Not only is our model trained on a different class distribution, it is not provided any object labels during training. Thus we compare our approach to other label-free representation learning approaches~\citep{berthelot2018acai, donahue2016bigan, caron2018deepcluster}. We also compare with methods in unsupervised few-shot learning such as CACTUs~\cite{hsu2018cactus}, AAL~\cite{antoniou2019assume} and UMTRA~\cite{khodadadeh2019umtra} that also use no class labels until test time. These methods do still benefit from training on the same class distribution used in testing, however, we also swap the training datasets to address any differences in dataset size. We still include VAE baselines from Section~\ref{sec:novel_classification} as well as a Random CNN as a baseline embedding function.

\subsubsection{Few-shot classification on Omniglot}
The Omniglot~\citep{Lake2015bpl} dataset contains 50 alphabets, 1623 unique character types, each with 20 examples and is presented as both a greyscale image and a stroke drawing. We use the same train-test split as~\citet{vinyals2016matching} along with randomly sampled episodes. Results are presented in Table~\ref{tab:omniglot_results} Experiments using the more challenging Lake split where episodes are sampled within alphabet, as proposed by \citet{Lake2015bpl}, are in Appendix \ref{appendix:lake_split} and random seed experiments in Appendix \ref{appendix:seeding}.

Results from training only on Omniglot~\citep{Lake2015bpl} are also presented to demonstrate effectiveness without the larger Quickdraw\citep{jongejan2016quickdraw} dataset. No significant improvements were observed using the deeper ResNet12\citep{oreshkin2018tadam} architecture; additional results are in Appendix \ref{appendix:full_omniglot_table}.

\subsubsection{Few-shot classification on mini-ImageNet}
The mini-ImageNet~\citep{vinyals2016matching} dataset consists of 100 classes each with 600 examples. The split proposed by~\citet{ravi2016optimization} is used, where sets of 64-16-20 classes are used for training, validation and test. As noted earlier, any examples in the Sketchy dataset that are also present in the mini-ImageNet test were removed by filtering the synset (and children synset) IDs ensuring train and test classes are disjoint. Unlike with Quickdraw, the total amount of training data is comparable with the Sketchy~\citep{Sangkloy2016sketchy} dataset. Classification results on mini-ImageNet are shown in Table~\ref{tab:mini-imagenet_results}.

\subsection{Pixel loss ablation}
\input{sections/tables/tab_alpha_sweep}
We ablate pixel loss coefficient $\alpha_\text{max}$ to quantify it's impact on the observed representation using the Omniglot task (Table \ref{tab:alpha_sweep}). There is a substantial improvement in few-shot classification when $\alpha_\text{max}$ is non-zero. $\alpha_\text{max}$= 0.50 achieves the best results, while it trends downwards when $\alpha_\text{max}$ approaches to 1.0.

\begin{figure}[t]
    \centering
    \includegraphics[trim=6.1cm 0.4cm 7cm 0cm,clip,width=0.48\textwidth]{figures/compositionality/component_arrangements.pdf}
    \caption{UMAP clustering of different component arrangements.}
    \label{fig:compositionality_component_arrangements}
\end{figure}

\subsection{Classification discussion}
Like humans, machine learning systems appear to benefit through using \modelembedding{}s. \model{} based classification consistently outperforms other label-free representation learning methods. By decoding image embeddings as a sketch motor program, the representation encodes how to "draw" a representative sketch of it's input. By understanding a visual input as a sketch the embedding must explicitly understanding individual components due to their contiguous definition by sequential pen movements through time. Pixel based methods may be less aware of individual components as they generate all pixels at once and use no other input-output correspondence. The contrastive loss also performs better than pixel-based methods but may not experience the full benefit of sketching as it only requires agreement between image and sketch embeddings rather than encapsulating the full drawing in an image embedding.

\modelembedding{}s trained using sketch reconstruction also show to be a more generalized representation. Our method achieves the highest classification accuracy on the Omniglot~\citep{Lake2015bpl} challenge and is competitive with the state-of-the-art on the mini-ImageNet~\citep{vinyals2016matching} benchmark. By knowing how to draw, our model can sketch an unidentified object, save a structured and salient representation that can be identified later at test time. We believe this phenomenon, combined with the more explicit compositional understanding, allows \modelembedding{}s to be more informative outside of training examples, classes and even datasets (Figure~\ref{fig:few_shot_samples}. 

==> sections/compositionality.tex <==
% !TEX root = ../main.tex
\begin{figure}[t]
    \centering
    \includegraphics[trim=6.1cm 0.2cm 7cm 0cm,clip,width=0.48\textwidth]{figures/compositionality/component_arrangements.pdf}
    \caption{UMAP clustering of different component arrangements.}
    \label{fig:compositionality_component_arrangements}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[trim=6.1cm 0.4cm 7cm 0cm,clip,width=0.48\textwidth]{figures/compositionality/spatial_relationships.pdf}
    \caption{Recovering spatial variables by UMAP clustering.}
    \label{fig:compositionality_spatial_relationships}
\end{figure}

\section{Properties of \modelembedding{}s}
\label{sec:compositionality}
We hypothesize that reproducing a sketch drawing rather than a pixel-based approach requires the preservation of more structural information due to sequential RNN generation. By learning in this manner, \model{}s are aware of spatial properties and the composition of elements in image space. We examine this compositionality through several comparisons of \model{}s with those generated by a Conv-VAE.

\subsection{Arrangement of image components}
Components of a sketch are often typically drawn contiguously through time. Knowing how to draw should necessitate identifying individual components and repeatedly plotting them. To test this, we construct image examples containing different arrangements of multiple objects in image space.  We then embed these examples and project into 2D space using UMAP~\citep{mcinnes2018umap} to visualize their organization. The leftmost panel of Figure \ref{fig:compositionality} exhibits non-synthetic classes with duplicated components; snowmen with circles and televisions with squares. The next 2 panels of contain synthetic examples with variations that maintain a similar silhouette. \modelembedding{}s are the most distinguishable and are easily separated by clustering. The pixel-based Conv-VAE is the least distinguishable while the sketch-supervised contrastive model performs well in the far right case but poorly in the other two. By learning to draw, \modelembedding{}s retain a stronger component awareness that is useful for understanding compositional image inputs.

\subsection{Recovering spatial relationships.}
We examine the how the underlying variables of angle, distance or size are captured by the studied embedding functions. We construct and embed examples changing each of the variables of interest. The embeddings are again grouped by a 2D projection in Figure \ref{fig:compositionality_spatial_relationships} using the UMAP~\citep{mcinnes2018umap} algorithm. When clustered, the 2D projection of \model{}s recovers the variable of interest as a mostly linear manifold in 2D space; the contrastive sketch embedding replicates this in some degree while the pixel-based Conv-VAE is visibly clustered and non-linear. We show that being able to produce a sketch requires awareness of the explicit spatial relationships between components which is then better preserved in latent representations.

\subsection{Conceptual composition}
\begin{figure}[t]
    \centering
    \includegraphics[trim=0cm 0cm 21.2cm 11.5cm,clip,width=0.48\textwidth]{figures/compositionality/conceptual_composition.pdf}
    \caption{Conceptual composition examples.}
    \label{fig:compositionality_conceptual_composition}
\end{figure}

Finally, we explore the use of \modelembedding{}s for composing embedded concepts. We embed examples of simple shapes such as a square or circle as well as more complex examples like a snowman or mail envelope and perform arithmetic in the latent space. Surprisingly, upon decoding the \modelembedding{} vectors we recover intuitive sketch generations. For example, if we subtract the embedding of a circle from snowman and add a square our decoded image is a stack of boxes. We present examples in Figure~\ref{fig:compositionality_conceptual_composition}. The Conv-VAE does not  produce any sensible decodings while \model{} decodes a number of interesting examples transforming circle and square based shapes to a number of other silhouettes.

By learning a sequence generating model we recover the well known natural language phenomenon that allows word embeddings to be composed in manners such as "King - Man + Woman = Queen"~\citep{linearwordanalogies} while no such behaviour is observed for pixel-based embeddings. Our method now defines an natural language embedding property for visual image media . DeepSVG~\citep{carlier2020deepsvg} demonstrates a similar phenomenon but treats embeddings as properties that can be muted or emphasized and is defined for scalable vector graphics (SVGs).

==> sections/discussion.tex <==
% !TEX root = ../main.tex
% \section{Discussion}
% \label{sec:discussion}
% \subsection{Version 2}

% \paragraph{Learning to draw for classification.} 
% \model{} demonstrates strong classification accuracy generalization across new examples and datasets. While Contrastive is competitive in Quickdraw classification, the easiest benchmark, it does not maintain this performance on more difficult tasks with natural images.
% The gap between Contrastive and our \model{} demonstrate that simply including the stroke information during training is not enough to achieve the best performance.
% This result suggests that the contrastive objective is not as informative as our autoregressive generative objective, which aims to produce a quality sketch in an one-shot manner. Visualizations also confirm that our \modelembedding{} generalizes well to novel examples and classes from the source domain (see Figure~\ref{fig:seen_sketches}), as well as new target data domains (see Figure~\ref{fig:few_shot_samples}).
% We observe that sketches of mini-ImageNet examples only capture the general structure of the object which may explain the lower absolute accuracy on the benchmark. 
% Just as humans can recognize and draw an unfamiliar object, 
% learning to sketch is a useful task for learning novel visual concepts.


% \MR{do you mean the diff between Quick draw and miniImageNet?} 
% and it is clear that \model{}'s performance is not only due to the use of sketch motor programs. 
% While a contrastive loss builds agreement between two domains it does not require the latent embedding to fully capture the informative sketch domain. 

% However, a generative model must fully encode this sketch information in order to produce a quality sketch and satisfy the training objective. We see that \model{} does capture this information and produces quality sketches of novel examples and classes from the training dataset (Figure~\ref{fig:seen_sketches}). 
% Furthermore, by learning to sketch one dataset it is able to infer a sketch of novel Omniglot~\citep{Lake2015bpl} and mini-ImageNet~\citep{vinyals2016matching} datasets, produce quality sketches (Figure~\ref{fig:few_shot_samples}) and effectively facilitate classification. 
% relate it to other instances 
% and then identify them as a group, 


% \paragraph{Learning emergent properties.}
% In Section~\ref{sec:compositionality}, \modelembedding{}s exhibit interesting emergent properties: They are aware of discrete image components and the spatial separation between them in 2D space. As we see in Figure \ref{fig:compositionality_component_arrangements} and \ref{fig:compositionality_spatial_relationships}, sketching the 4 strokes of a square versus the many small segments to approximate a circle are easily separable in a motor representation. 
% As these image components are drawn contiguous through time and separated by lifted pen states, the model learns to group the input pixels together as abstract elements to be drawn together. 
% Finally, the model must also understand spatial offsets between these components in order to produce the $\Delta \bm{x} $ and $ \Delta \bm{y}$ values to satisfy the training objective.

% The conceptual composition of \modelembedding{}s portrays a phenomenon appealing to human intuition. In the simple examples demonstrated, the concept of a ``stack of boxes'' can be gained by embedding such an image but can also be constructed through the embeddings of a snowman, circle and a square. This emergent linear compositional property has been discovered in the continuous bag-of-word embeddings~\citep{mikolov2013cbow} in natural language learning and more recently has been demonstrated in some vision models for human faces~\citep{bojanowski2017optimizing, shen2020interpreting}. It has also been recently observed in DeepSVG~\citep{carlier2020deepsvg} for vector graphics learning.


==> sections/generation.tex <==
% !TEX root = ../main.tex
\section{Sketch Generation}
While we the focus of our paper is on representation learning, \model{} is still a visually appealing generative model. In Figure~\ref{fig:seen_samples} we present sketches of unseen examples of seen classes. Generations of unseen classes and datasets were presented in Figure~\ref{fig:few_shot_samples}. While the novel image sketches are not as impressive as those from the Quickdraw~\citep{jongejan2016quickdraw} and Omniglot~\citep{Lake2015bpl}, it is a far more challenging task with considerably less data. It is worth noting that while the sketches often may only capture the general shape of the subject in the image, that is sufficient understanding to drive our impressive classification performance in Section~\ref{sec:classification}. We would classification performance to improve alongside generation quality given more data.

\begin{figure}[t]
    \centering
    \includegraphics[trim=0.05cm 0.05cm 7cm 6.7cm,clip,width=0.48\textwidth]{figures/seen_samples.pdf}
    \caption{Sketches of unseen examples}
    \label{fig:seen_samples}
\end{figure}


==> sections/old/compositionality.tex <==
% !TEX root = ../main.tex

\vspace{-0.1in}
\section{Properties of \model{}s}
\vspace{-0.1in}
\label{sec:compositionality}
We hypothesize that reproducing a sketch drawing rather than a pixel-based approach requires the preservation of more structural information due to sequential RNN generation. By learning in this manner, \model{}s are aware of spatial properties and the composition of elements in image space. We examine this compositionality through several comparisons of \model{}s with those generated by a Conv-VAE.

% \vspace{-0.1in}
% \paragraph{Spatial component relation}
% We construct images that contain the same set of objects but with different spatial relations to test sensitivity to object arrangements in image space.
% We embed these examples with both generative models then project into 2D space using UMAP \citep{mcinnes2018umap}.
% We also apply a simple linear classifier trained on 100 examples and tested on 200 to predict the class of each embedding. In the first 2 panels of Figure \ref{fig:compositionality}\textbf{A}, we see that the \model{}s are more informative than those of the VAE as they are easily separated and are classified with higher accuracy shown in the bottom left. The rightmost panel of Figure \ref{fig:compositionality}\textbf{A} exhibits non-synthetic classes with duplicated shapes; snowmen with circles and televisions with squares. This shows that learning to draw facilitates an understanding of pen actions that vary for different, but visually similar shapes.

% \vspace{-0.1in}
% \paragraph{Latent variable recovery}
% Drawing also builds awareness of canvas localization and subject scale. We examine how varying an underlying latent variable is captured in embeddings, by constructing images that vary in angle, distance or size. The embeddings are visualized by 2D projection in Figure \ref{fig:compositionality}\textbf{B} and used for a regression task with a simple linear model. $R^2$ values are in the bottom right; once again 100 training examples and 200 test examples are used. The 2D projection of \model{}s arranges the examples in each task along an axis corresponding to the latent variable and is far more successful in the regression task when compared to a Conv-VAE.

% \vspace{-0.1in}
% \paragraph{Conceptual composition}
% Finally, we explore conceptual composition using \model{}s (Figure \ref{fig:compositionality}\textbf{C}) by embedding different Quickdraw examples then performing arithmetic with the latent vectors. By subtracting a circle embedding and adding a square embedding from a snowman composed of stacked circles, we produce stacked boxes. This property of vector arithmetic is reminiscent of language representations and is evidenced in analogies like King - Man + Woman = Queen~\citep{linearwordanalogies}. Surprisingly, this property is present in \model{} and is not shown in the pixel-based VAE embeddings.

\vspace{-0.1in}
\paragraph{Component arrangements} 
We construct examples that contain the same set of objects but in different arrangements to test sensitivity to component arrangement and composition in image space. We then embed these examples with both generative models and project into 2D space using UMAP~\citep{mcinnes2018umap} to visualize their organization.  In the first 2 panels of Figure \ref{fig:compositionality}-A, we see that the \model{}s are easily separated in unsupervised clustering. The rightmost panel of Figure \ref{fig:compositionality}-A exhibits non-synthetic classes with duplicated shapes; snowmen with circles and televisions with squares. With these results, we demonstrate the greater component level awareness of \model{}s. The 4 rearranged shapes and the nested circle and squares have similar silhouettes that are difficult to differentiate to a conventional pixel loss. To \model{}s, the canvas offset and different drawing sequence of each shape make them substantially different in embedding space.

\vspace{-0.1in}
\paragraph{Spatial relationships}
Drawing also builds awareness of relevant underlying variables, such as spatial relationships between components of the image. We examine the degree to which the underlying variables of angle, distance or size are captured by the embedding, by constructing images that vary along each dimension respectively. The embeddings are again grouped by a 2D projection in Figure \ref{fig:compositionality}-B using the UMAP~\citep{mcinnes2018umap} algorithm. When clustered, the 2D projection of \model{}s arranges the examples along an axis corresponding to the latent variable compared to the Conv-VAE embeddings which is visibly non-linear and arranges in clusters. This clear axis-alignment suggests a greater level of latent variable disentanglement in the \model{}s.

\vspace{-0.1in}
\paragraph{Conceptual composition}
Finally, we explore concept space composition using \model{}s (Figure \ref{fig:compositionality}-C) by embedding different Quickdraw examples then performing arithmetic with the latent vectors. By subtracting a circle embedding and adding a square embedding from a snowman composed of stacked circles, we produce stacked boxes. This property of vector arithmetic is reminiscent of language representations, as evidenced in analogies like King - Man + Woman = Queen~\citep{linearwordanalogies}. Our results indicate that this property is captured to a greater degree in \model{} than in the pixel-based VAE embeddings. Composing \model{}s produces decoded examples that appeal to our intuitive conceptual understanding while the VAE degrades to blurry, fragmented images. We provide more examples of the setup in Figure \ref{fig:compositionality}-C as well as additional classes in Appendix \ref{appendix:more_concept_comp}.

==> sections/old/conclusion.tex <==
% !TEX root = ../main.tex
\section{Conclusion}
\vspace{-0.1in}
Learning to draw is not only an artistic pursuit but drives a distillation of real-world visual concepts. We present a generalized drawing model capable of producing accurate sketches and visual summaries of open-domain natural images. While sketch data may be challenging to source, we show that training %by our method 
to draw either sketch or natural images can generalize for downstream tasks, not only within each domain but also well beyond the training data. 
More generally research in this direction may lead to 
%We bring new, and 
more lifelike image understanding inspired by how humans communicate visual concepts.

==> sections/old/drawing_imitation.tex <==
% !TEX root = ../main.tex
\vspace{-0.1in}
\section{Drawing Imitation Experiments}
\vspace{-0.1in}
\label{sec:drawing_imitation}
In this section, we introduce our experiments on training
\drawmodel{} using two sketching datasets. The first is based on pure stroke-based drawings, and the second consists of natural image and drawing pairs.

\input{sections/tab_omniglot_main}

\vspace{-0.1in}
\paragraph{Quickdraw: Stroke-based image sketching}

The Quickdraw~\citep{jongejan2016quickdraw} dataset consists of 345 classes of each with 70,000 examples, produced by human players participating in the game ``Quick, Draw!''. Examples from the Quickdraw dataset are shown in Figure~\ref{fig:quickdraw_samples}. The input image $\bm{x}$ is a direct rasterization of the drawing data $\bm{y}$.
300 of 345 classes are randomly selected for training; $\bm{x}$ is rasterized to a resolution of $28 \times 28$ and stroke labels $\bm{y}$ padded up to length $T = 64$. Any drawing samples exceeding this length were discarded. Note that this an unsupervised representation learning approach, as no class information is used by the system. Data processing procedures and class splits are in Appendix \ref{appendix:data_processing}.

\vspace{-0.1in}
\paragraph{Sketchy: Open domain natural image sketching}
We further extend our stroke-based generation model on open domain natural images. Here, the input is an RGB photo, and the output is a human drawing which does not align with the photo precisely and also does not match with the low-level image details. This is a novel setting, as prior efforts by~\citet{ha2017sketchrnn,chen2017pix2seq,learn2sketchcycle} have only applied their sketch RNN models on the Quickdraw dataset or natural images with only two object classes (shoe/chair) and scrubbed backgrounds~\citep{sketchshoe}. Learning to sketch open domain natural images is very challenging as it requires the model to identify the subject and filter unnecessary details not present in the sketch. At test time, we further challenge our method by evaluating on unseen data distributions necessitating generalization over natural images. 

For this task we use the Sketchy dataset~\citep{Sangkloy2016sketchy} which consists of ImageNet images paired with vector sketches for a total of 56k examples after processing. Sketches are stored as SVGs with timestamps preserving their original drawing sequence which we adapt by sampling paths in this order. Images are also centered, padded and resized to resolution $84 \times 84$ (see Figure \ref{fig:sketchy_samples}). We fix the maximum sequence length to $T=100$, and use all 125 categories but remove classes that have overlapping child synsets with the test classes of mini-ImageNet~\citep{vinyals2016matching}. This enables testing on mini-ImageNet without any alterations to the benchmark. Once again this is an unsupervised learning formulation.

\vspace{-0.1in}
\subsection{Results and visualizations}
\vspace{-0.05in}
Figure \ref{fig:quickdraw_imitation} shows drawings conditioned on sketch image inputs. There is little noticeable drop in quality when we sample sketches from unseen classes compared to those it has seen before. Figure \ref{fig:open-domain_natural_image_sketch} shows examples of sketches generated from natural images. While they are not fine-grained renditions, these sketches clearly demonstrate \drawmodel{}'s ability to capture key components of seen and unseen classes. The model effectively isolates the subject in each natural image and captures the circular and square shapes in the cakes and storefronts respectively. Even with the challenging lion images, it identifies the silhouette of the laying lion despite low contrast and appropriately localizes the one on the mountainside.

Unlike pixel-based auto-encoder models, our sketches do not follow the exact pose of the original strokes, but rather capture a general notion of component groupings. In the basketball example of Figure~\ref{fig:quickdraw_imitation}, the lines are not a good pixel-wise match to those in the original image yet they are placed in sensible relative positions. Weaker examples are presented in the last row of Figure~\ref{fig:quickdraw_imitation} and \ref{fig:open-domain_natural_image_sketch}; regardless, even poorer examples still capture some structural aspects of the original image. Implementation details can be found in Appendix \ref{appendix:implementation_details}.

% In later sections we explore the uses of \model{}s and fix models for all downstream tasks.
In later sections we explore the uses of \model{}s, no stroke data is used beyond this point.


==> sections/old/drawingvis.tex <==
\begin{figure}[t]
    \vspace{\topbreak{}}
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=1\textwidth]{primaryfigs/drawing_imitation/sketch_seen_to_sketch_box_fail.png}
        
        \vspace{0.1cm}
        
        \includegraphics[width=1\textwidth]{primaryfigs/drawing_imitation/sketch_unseen_to_sketch_box_fail.png}
        \caption{Sampled generated drawings of Quickdraw examples. Weaker drawings boxed in red.}
        \label{fig:quickdraw_imitation}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=1\textwidth]{primaryfigs/drawing_imitation/natural_seen-to-sketch_fail.png}
        
        \vspace{0.1cm}
        
        \includegraphics[width=1\textwidth]{primaryfigs/drawing_imitation/natural_unseen-to-sketch_fail.png}
        \caption{Sampled drawings of mini-ImageNet examples. Weaker drawings boxed in red.}
        \label{fig:open-domain_natural_image_sketch}
    \end{minipage} 
    \vspace{-0.15in}
\end{figure}


==> sections/old/few-shot_classification.tex <==
\vspace{-0.1in}

\section{Few-shot Classification using \model{}}
\label{sec:fsc}
\vspace{-0.1in}
We would like to assess the benefits of learning to draw by performing few-shot classification with our learned embedding space. Examining performance on discriminative tasks reveals that learning
to imitate sketches allows the embeddings to capture salient information of novel object classes. Below we describe our few-shot classification procedure and summarize results on the Omniglot~\citep{Lake2015bpl} and mini-ImageNet benchmarks~\citep{vinyals2016matching}.

\input{sections/tab_miniimagenet_main}

\vspace{-0.1in}
\paragraph{Comparison to unsupervised few-shot classification}
In unsupervised few-shot classification, a model is not provided with any class labels during meta-training, until it is given a few labeled examples ("shots") of the novel classes at meta-test time.
While our model is provided a "target"---a sequence of strokes---during training, it is not given any class information. Therefore, we propose that the presented sketch imitation training, though it uses sketch sequences, is comparable to other class-label-free representation learning approaches~\citep{berthelot2018acai, donahue2016bigan, caron2018deepcluster}
and the learned \model{}s can be applied to unsupervised few-shot classification methods. 

In our experiments, we compare to previous unsupervised few-shot learning approaches: CACTUs~\citep{hsu2018cactus}, AAL~\citep{antoniou2019assume}, and UMTRA~\citep{khodadadeh2019umtra}. These methods create pseudo-labels during meta-training using either clustering or data augmentation. As additional baselines, a Conv-VAE~\citep{vae} and a random CNN are also included, both using the same Conv4 backbone.

\vspace{-0.1in}
\paragraph{Few-shot experimental setup}
% The CNN encoder of \drawmodel{} is used as an embedding function combined with a linear classification head to perform few-shot classification. 
The CNN encoder of \drawmodel{} is used as an embedding function combined with a linear classification head to perform few-shot classification; encoder weights are fixed and no sequential data is used during few-shot training or evaluation.
The embedding is made deterministic by taking the mean of the random normal latent space $\bm{z}$ and discarding the variance parameter from the encoder. Otherwise, the conventional episodic setup for few-shot classification is used; each episode consists of a labeled "support" set of $N \times K$ (N-way K-shot) embeddings and an unlabeled "query" set. The linear classification head is trained on the labeled support set and evaluated on the query set.

\vspace{-0.1in}
\subsection{Few-shot classification on Omniglot}
\vspace{-0.05in}
The Omniglot~\citep{Lake2015bpl} dataset contains 50 alphabets, 1623 unique character types, each with 20 examples and is presented as both a greyscale image and a stroke drawing. We use the same train-test split as~\citet{vinyals2016matching} along with randomly sampled episodes. Experiments using the more challenging Lake split where episodes are sampled within alphabet, as proposed by \citet{Lake2015bpl}, are in Appendix \ref{appendix:lake_split} and random seed experiments in Appendix \ref{appendix:seeding}.

To ensure a fair comparison with other few-shot classification models, we use the same convolutional encoder (Conv4) as~\citet{vinyals2016matching}. Results from training only on Omniglot~\citep{Lake2015bpl} are also presented to demonstrate effectiveness without the larger Quickdraw\citep{jongejan2016quickdraw} dataset. No significant improvements were observed using the deeper ResNet12\citep{oreshkin2018tadam} architecture; additional results are in Appendix \ref{appendix:full_omniglot_table}.

All of our methods out-perform the previous state-of-the-art on the unsupervised Omniglot benchmark (Table \ref{tab:omniglot_results}). The Quickdraw trained model surpasses supervised MAML~\citep{finn2017maml}, and is on par with a supervised ProtoNet~\citep{snell2017prototypical} model
% despite training on an entirely different distribution of sketches rather than handwritten characters. We report both the best seed and an average of 15 random seeds. The demonstrated approach excels in higher-shot settings and also manages to match the supervised ProtoNet model in the 5-shot regime. 
, especially in the 5-shot settings.
Both baselines, a Conv-VAE and a random CNN, perform well compared to other unsupervised methods.

\vspace{-0.1in}
\subsection{Few-shot classification on mini-ImageNet}
\vspace{-0.05in}
We extend our investigation and assess \model{}s for the classification of natural images in the mini-ImageNet benchmark~\citep{vinyals2016matching}. The same CNN encoder model from the natural image sketching task is used to match the visual domain of the examples we hope to classify. 
% \RZ{Can cut next sentence} By training \drawmodel{} on the Sketchy~\citep{Sangkloy2016sketchy} dataset that maps ImageNet photos to a stroke drawing label, we teach \drawmodel{} to summarize the natural image domain.

The mini-ImageNet~\citep{vinyals2016matching} dataset consists of 100 classes each with 600 examples. The setup proposed by~\citet{ravi2016optimization} is used, where the classes are split 64-16-20 for training, validation and test. As noted earlier, any examples in the Sketchy dataset that are also present in the mini-ImageNet test were removed by filtering the synset (and children synset) IDs ensuring train and test classes are disjoint.

Classification results on mini-ImageNet are shown in Table~\ref{tab:mini-imagenet_results}. Natural image classification is a far more challenging problem. Learning to reconstruct pixels of an image actually worsens our results; the trained Conv-VAE is outperformed by the VAE with random weights. However, sketch reconstruction is still a valuable task; our models are competitive while our best model out-performs previous state-of-the-art unsupervised methods on few-shot settings. A full table is in Appendix \ref{appendix:full_mii_table}, seeding results are in Appendix \ref{appendix:seeding}.

\vspace{-0.1in}
\subsection{Sketching to learn class-identifiable information}
\vspace{-0.05in}
Existing sketch works have focused on generating better drawings or unifying sketches with other image domains. We present a new paradigm: using sketching as an auxiliary task to learn visual content. Only by training a drawing model that can sketch general image inputs are we able to transfer the learned understanding to new data distributions. By considering the stroke distribution of the Quickdraw dataset, we are able to interpret image inputs from the separate Omniglot dataset and tackle the few-shot classification task with surprising accuracy.

While the natural image sketching task is challenging and does not always produce high-fidelity results, it still learns useful visual information. By training on the Sketchy dataset, we learn how to draw other data distributions for which no sequential stroke data exists. Then, by knowing how to sketch this mini-ImageNet data we are able to produce distinguishable embeddings that enable competitive few-shot classification performance.

\begin{figure}[t]
    \vspace{\topbreak{}}
    \centering
    \includegraphics[trim=5.45cm 4.25cm 5.1cm 3.53cm,clip,width=0.98\textwidth]{primaryfigs/compositionality_figs/composed_compositionality_figure_6.pdf}
    \caption{Experiments exploring properties of \model{}s. Examples colored for understandability only.}
    \label{fig:compositionality}
    \vspace{-0.15in}
\end{figure}

\vspace{-0.1in}
\paragraph{Varying weighting of pixel-loss}
For both settings we sweep the pixel loss coefficient $\alpha_\text{max}$ to ablate its impact on model performance on the Omniglot task (Table \ref{tab:alpha_values}). There is a substantial improvement in few-shot classification when $\alpha_\text{max}$ is non-zero. $\alpha_\text{max}$= 0.50 achieves the best results, and the trend goes downward when $\alpha_\text{max}$ approaches to 1.0, i.e. the weighting for $\mathcal{L}_{\text{stroke}}$ goes to 0.0. This is reasonable as the training of \drawmodel{} is more stable under the guidance of ground truth strokes.


==> sections/old/generative_evaluation.tex <==

\vspace{-0.1in}
\section{One-Shot Generation}
\vspace{-0.1in}
\label{sec:fsg}
To evaluate the 
sketches generated by our model, we make qualitative comparisons to other one-shot generative models and quantitatively assess our model through visual classification via a ResNet101 ~\citep{He2016resnet}. In this section, all models use the ResNet12~\citep{oreshkin2018tadam} backbone.
\begin{figure}[t]
    \vspace{\topbreak{}}
    \centering
    \includegraphics[trim=0cm 0.22cm 0cm 0.2cm,clip,width=0.75\textwidth]{primaryfigs/generation/generation-other-papers.png}
    \caption{One-shot Omniglot generation compared to ~\citet{oneshotgen, fewshotgen}.}
    \label{fig:otherpapergenerations}
    \vspace{-0.15in}
\end{figure}

\vspace{-0.1in}
\paragraph{Qualitative comparisons} We compare \drawmodel{} one-shot generations of Omniglot characters with examples from other few-shot~\citep{fewshotgen} and one-shot~\citep{oneshotgen} approaches (Figure \ref{fig:otherpapergenerations}). In the settings shown, none of the models have seen any examples from the character class, or the parent alphabet. Furthermore, the drawer has seen no  written characters during training and is trained only on the Quickdraw dataset. Visually, our generated images better resemble the support examples and the variations by stretching and shifting strokes better preserves the semantics of each character. Generations in pixel space may disrupt strokes and alter the character to human perception. This is especially true for written characters as they are frequently defined by a specific set of strokes instead of blurry clusters of pixels.

\vspace{-0.1in}
\paragraph{Quantitative evaluation of generation quality}
Evaluating generative models is often challenging. Per-pixel metrics like in ~\citet{fewshotgen, oneshotgen} may penalize generative variance that still preserves meaning. We propose an Inception Score \citep{inception} inspired metric to quantify class-recognizability and generalization of generated examples. We train two separate ResNet classifiers~\citep{He2016resnet}, each on a different set of 45 Quickdraw classes. One set was part of the training set of \drawmodel{} (referred to as ``seen'') and the other set was held out during training (referred to as ``unseen''). We then have \drawmodel{} generate one-shot sketches from each set and have the corresponding classifier predict a class. The accuracy of the classifier on generated examples is compared with its training accuracy in Table \ref{tab:generative_scores}. For a ResNet classifier, \drawmodel{} generations are more recognizable for both classes seen and unseen classes.

\input{sections/tab_resnet_score}



==> sections/old/impact_statement.tex <==
% !TEX root = ../main.tex
\section*{Broader Impact}
In this paper we aim to learn general neural embeddings for compositional drawings. We discover that the learned embedding is very informative in terms of recognizing novel objects, even though it has never seen a class label. We show that it achieves amazing performance on few-shot learning, due to its capability of transform rich input data into abstract sketch space. One potential application is to help general purpose home robotics so that they can learn new skills with a few demonstrations. The automatic sketch technology we develop can also promote the development of AI arts and assistive technology for handicaps, for examples. On the other hand, we believe that the risk and unintended impact of our algorithm is no greater than other general AI technologies. For instance, although few-shot learning itself can be used in surveillance technologies, it is no different from hiring a human to perform the same task. Ultimately, unethical impact comes from the hands of unethical people, not technology itself.

==> sections/old/intro.tex <==
% !TEX root = ../main.tex
\vspace{-0.15in}
\section{Introduction}
\vspace{-0.1in}

Upon encountering a novel concept, such as a six-legged turtle, humans can quickly generalize this concept by composing a mental picture. The ability to generate drawings greatly facilitates communicating new ideas. This dates back to the advent of writing, as many ancient written languages are based on logograms, such as Chinese hanzi and Egyptian hieroglyphs, where each character is essentially a sketch of the object it represents. %And, we have all seen how a complicated concept can be conveyed by a few simple strokes.
We often see complex visual concepts summarized by a few simple strokes.

Inspired by the human ability to draw, recent research has explored the potential to generate sketches using a wide variety of machine learning models, ranging from hierarchical Bayesian models~\citep{Lake2015bpl}, to more recent deep autoregressive models~\citep{draw,ha2017sketchrnn,chen2017pix2seq} and generative adversarial nets (GANs)~\citep{photosketch}. It is a natural question to ask whether we can obtain useful intermediate representations from models that produce sketches in the output space, as has been shown by other generative models~\citep{sparseenergy,vae,gan,donahue2016bigan,context}. Unfortunately, a hierarchical Bayesian model suffers from prolonged inference time, while other current sketch models mostly focus on producing drawings in a closed set setting with a few classes~\citep{ha2017sketchrnn,chen2017pix2seq}, or on improving log likelihood at the pixel level~\citep{oneshotgen}. Leveraging the learned representation from these drawing models
remains a rather unexplored topic.

In this paper, we pose the following question: \textit{Can we learn a generalized embedding function that captures salient and compositional features by directly imitating human sketches?} The answer is affirmative. In our experiments we develop \drawmodel{}, an RNN-based sketch model trained to map grayscale and natural image pixels to the sketch domain. It is trained on hundreds of classes without the use of class labels to learn a robust drawing model that can sketch diverse and unseen inputs. 
% We evaluate the latent ``\model{}'' on unsupervised few-shot classification, and achieve state-of-the-art performance on the Omniglot \citep{Lake2015bpl} dataset. We then explore how the embeddings depend on image components and their spatial relations. As well, we investigate the generative variance and recognizability of samples in one-shot generation. 
We demonstrate salience by achieving state-of-the-art performance on the Omniglot few-shot classification benchmark and visual recognizability in one-shot generations. Then we explore how the embeddings capture image components and their spatial relationships to explore image space compositionality and also show a surprising property of conceptual composition.

We then push the boundary further by applying our sketch model to natural images---to our knowledge, we are the first to extend stroke-based autoregressive models to produce drawings of open domain natural images. We train our model with adapted SVG images from the Sketchy dataset~\citep{Sangkloy2016sketchy} and then evaluate the embedding quality directly on unseen classes in the mini-ImageNet task for few-shot classification~\citep{vinyals2016matching}. Our approach is competitive with existing unsupervised few-shot learning methods~\citep{hsu2018cactus,khodadadeh2019umtra,antoniou2019assume} on this natural image benchmark.  In both the sketch and natural image domain, we show that by learning to draw, our methods generalize well even across different datasets and classes.

\begin{figure}[t]
    \vspace{\topbreak{}}
    \centering
    \includegraphics[width=0.98\textwidth]{primaryfigs/figure1_short.pdf}
    \caption[]{
    \textbf{A:} A natural or sketch pixel image is passed into the CNN encoder to obtain Gaussian \model{} $z$, which is concatenated with the previous stroke $y_{t-1}$ as the decoder input at each timestep to generate $y_t$. \textbf{B+C:} Downstream tasks performed after training is complete.}
    \label{fig:1_hlsetup}
    \vspace{-0.15in}
\end{figure}

==> sections/old/model.tex <==
% !TEX root = ../main.tex

\begin{figure}[t]
    \vspace{\topbreak{}}
    \centering
    \label{fig:dataset_examples}
    \begin{subfigure}{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{primaryfigs/dataset_samples/sketchy_samples.png}
         \caption{Sketchy samples}
         \label{fig:sketchy_samples}
     \end{subfigure}
     \begin{subfigure}{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{primaryfigs/dataset_samples/quickdraw_samples.png}
         \caption{Quickdraw samples}
         \label{fig:quickdraw_samples}
     \end{subfigure}
     \caption{Examples from Sketchy~\citep{Sangkloy2016sketchy} and Quickdraw~\citep{jongejan2016quickdraw} datasets. Sketchy examples are reshaped and padded to increase image--sketch spatial agreement.}
    \vspace{-0.15in}
\end{figure}

\vspace{-0.1in}
\section{Learning to Imitate Drawings}
\label{sec:model}
\vspace{-0.1in}
Here we describe learning to draw through sketch imitation. Our architecture is a generative encoder-decoder model with a CNN encoder for pixel images and an RNN decoder to output vector sketches as shown in Figure \ref{fig:1_hlsetup}. Unlike other drawing models that only train on a single or few classes~\citep{ha2017sketchrnn,chen2017pix2seq}, \drawmodel{} is not limited by class inputs and can sketch a wide variety of images. We also introduce a differentiable rasterization function for computing an additional pixel-based training loss.

% \vspace{-0.1in}
% \subsection{Input \& output representation}
% \vspace{-0.05in}
\vspace{-0.1in}
\paragraph{Input \& output representation}
Unlike SketchRNN which encodes drawing sequences, we learn an image embedding by mapping pixels to sketches, similar to~\citet{chen2017pix2seq}. Training data for this task (adopted from~\citet{ha2017sketchrnn}) consists of a tuple $(\bm{x}, \bm{y})$, where $\bm{x} \in \mathbb{R}^{H\times W \times C}$ is the input image and $\bm{y} \in \mathbb{R}^{T \times 5}$ is the stroke target. $T$ is the maximum sequence length of the stroke data $\bm{y}$, and each stroke $\bm{y}_t$ consists of 5 elements, $(\Delta_x, \Delta_y, s_1, s_2, s_3)$. The first 2 elements are horizontal and vertical displacements on the drawing canvas from the endpoint of the previous stroke. The latter 3 elements are mutually exclusive pen states: $s_1$ indicates the pen is on paper for the next stroke, $s_2$ indicates the pen is lifted, and $s_3$ indicates the sketch sequence has ended. $\bm{y}_0$ is initialized with (0, 0, 1, 0, 0) to start the generative process. Note that no class information is available while training.

% \vspace{-0.1in}
% \subsection{\model{} as a compositional encoding of images}
% \vspace{-0.05in}
\vspace{-0.1in}
\paragraph{\model{} as a compositional encoding of images}
We use a CNN to encode the input image $\bm{x}$ and obtain the latent space representation $\bm{z}$, as shown in Figure~\ref{fig:1_hlsetup}. To model intra-class variance, $\bm{z}$ is a Gaussian random variable parameterized by CNN outputs, similar to a VAE~\citep{vae}. Throughout this paper, we refer to $\bm{z}$ as the {\it \model{}}. In typical image representations the embedding is trained to classify object classes, or to reconstruct the input pixels. Here, since the \model{} is fed into an RNN decoder to produce a sequence of drawing actions, $\bm{z}$ is additionally encouraged to have a compositional understanding of the object structure, instead of just an unstructured set of pixel features. For example when drawing the legs of a turtle, the model must explicitly generate each leg instance. While pixel-based models suffer from blurriness and in generating the image at once, does not distinguish between individual components such as the legs, body and head. The loss of this component information by pixel models has been observed in GAN literature~\citep{gantutorial} which we propose is avoided by our sketching task.
% For instance, if the input image is a turtle with six legs, a regular CNN embedding will have salient features of legs in multiple places of the feature map. After an average pooling layer, it will only retain information about a leg-like feature but not how many legs are present and where they are positioned with respect to the canvas. The loss of compositional information of regular CNN embeddings is also observed in the GAN literature~\citep{gantutorial}. By contrast, the \drawmodel{} must preserve the information for drawing six distinct legs in order to succeed in the imitation task.

To accommodate the increased training data complexity by including hundreds of classes, we also upscale the size of our model in comparison to work by~\citet{chen2017pix2seq, ha2017sketchrnn, learn2sketchcycle}. The backbone is either a 4-layer CNN (Conv4)~\citep{vinyals2016matching} for consistent comparisons in the few-shot setting or a ResNet12~\citep{oreshkin2018tadam} which produces better drawing results. In comparison,~\citet{chen2017pix2seq} only use 2D convolution with a maximum of 8 filters.

\vspace{-0.1in}
\paragraph{RNN decoder}
The RNN decoder used in \drawmodel{} is the same as in SketchRNN~\citep{ha2017sketchrnn}. The decoder outputs a mixture density which represents the stroke distribution at each timestep. Specifically, the stroke distribution is a mixture of some hyperparameter $M$ bivariate Gaussians denoting spatial offsets as well as the probability of the three pen states $s_{1-3}$. The spatial offsets $\mathbf{\Delta} = (\Delta x, \Delta y)$ are sampled from the mixture of Gaussians, described by: (1) the normalized mixture weight $\pi_j$; (2) mixture means $\bm{\mu}_j=(\mu_x, \mu_y)_j$; and (3) covariance matrices $\Sigma_j$. We further reparameterize each $\Sigma_j$ with its standard deviation $\bm{\sigma}_j =(\sigma_x, \sigma_y)_j$ and correlation coefficient $\rho_{xy,j}$.
Thus, the stroke offset distribution is $p(\mathbf{\Delta}) =  \sum_{j=1}^{M}\pi_{j} \mathcal{N}(\bm{\Delta} \vert \bm{\mu}_j, \Sigma_j)$.


The RNN is implemented using a HyperLSTM~\citep{ha2013hypernetworks}; LSTM weights are generated at each timestep by a smaller recurrent ``hypernetwork'' to improve training stability. Generation is autoregressive, using $\bm{z} \in \mathbb{R}^D$, concatenated with the stroke from the previous timestep $\bm{y}_{t-1}$, to form the input to the LSTM. Stroke $\bm{y}_{t-1}$ is the ground truth supervision at train time (teacher forcing), or a sample $\bm{y'}_{t-1}$, from the mixture distribution output by the model during from timestep $t-1$.

\vspace{-0.1in}
\subsection{Learning} 
\vspace{-0.05in}
We train the drawing model in an end-to-end fashion by jointly optimizing three losses: a pen loss $\mathcal{L}_{\text{pen}}$ for learning pen states, a stroke loss $\mathcal{L}_{\text{stroke}}$ for learning pen offsets, and our proposed pixel loss $\mathcal{L}_{\text{pixel}}$ for matching the visual similarity of the predicted and the target sketch:
\vskip -0.8cm
\begin{align}
    \mathcal{L} = \mathcal{L}_{\text{pen}} + (1-\alpha)\mathcal{L}_{\text{stroke}} + \alpha \mathcal{L}_{\text{pixel}},
    \label{eq:loss}
\end{align}
\vskip -0.3cm
where $\alpha$ is a loss weighting hyperparameter. Both $\mathcal{L}_\text{pen}$ and $\mathcal{L}_\text{stroke}$ were in SketchRNN, while the $\mathcal{L}_\text{pixel}$ is our novel contribution to stroke-based generative models. Unlike SketchRNN, we do not impose a prior using KL divergence as we are not interested in unconditional sampling and it worsens quantitative results in later sections.

\vspace{-0.1in}
\paragraph{Pen loss} The pen-states predictions $\{s_1', s_2', s_3'\}$ are optimized as a simple 3-way classification with the softmax cross-entropy loss, $\mathcal{L}_{\text{pen}} = -\frac{1}{T}\sum_{t=1}^{T}\sum_{m=1}^3 s_{m, t}\text{log}(s'_{m,t})$.

\vspace{-0.1in}
\paragraph{Stroke loss} The stroke loss maximizes the log-likelihood of the spatial offsets of each ground truth stroke $\bm{\Delta}_t$ given the mixture density distribution $p_t$ at each timestep:
% \vskip -0.8cm
% \begin{align}
    $\mathcal{L}_{\text{stroke}} = -\frac{1}{T}\sum_{t=1}^{T} \log p_t(\bm{\Delta}_t)$.
% \end{align}
% \vskip -0.3cm

\vspace{-0.1in}
\paragraph{Pixel loss}
While pixel-level reconstruction objectives are common in generative models~\citep{vae,sae,draw}, we introduce a pixel-based objective for vector sketch generation. After decoding, a {\it differentiable rasterization} function $f_\text{raster}$ is used to map the sketch into a pixel image. $f_\text{raster}$ transforms a stroke sequence $\bm{y}$ into a set of 2D line segments ${(l_0, l_1), (l_1, l_2) \dots (l_{T-1}, l_{T})}$ where $l_t = \sum_{\tau=0}^t\bm{\Delta}_\tau$. It renders by fixing canvas dimensions, scaling and centering strokes before determining pixel intensity based on the $L_2$ distance between each pixel to lines in the drawing. Further details on $f_{\text{raster}}$ can be found in Appendix \ref{appendix:rasterization}. $f_\text{raster}$ is applied to both the prediction $\bm{y}'$ and ground truth $\bm{y}$, to produce two pixel images. Gaussian blur $g_{\text{blur}}(\cdot)$ is used to reduce strictness before computing the binary cross-entropy loss, $\mathcal{L}_{\text{pixel}}$:
\vskip -0.8cm
\begin{align}
    I &= g_{\text{blur}}(f_{\text{raster}}(\bm{y})), \quad
    I' = g_{\text{blur}}(f_{\text{raster}}(\bm{y}')), \quad
    \mathcal{L}_{\text{pixel}} = -\frac{1}{HW} \sum_{i=1}^H \sum_{j=1}^W I_{ij} \text{log}(I'_{ij}).
\end{align}
\vskip -0.3cm

\input{sections/drawingvis}

\vspace{-0.1in}
\paragraph{Curriculum training schedule}
We find that $\alpha$ (in Equation~\ref{eq:loss}) is an important hyperparameter that impacts both the learned embedding space and the generation quality of \drawmodel{}. A curriculum training schedule is used, increasing $\alpha$ to prioritize $\mathcal{L}_{\text{pixel}}$ relative to $\mathcal{L}_{\text{stroke}}$ as training progresses; this makes intuitive sense as a single drawing can be produced by many different stroke sequences but learning to draw in a fixed manner is easier. While $\mathcal{L}_{\text{pen}}$ promotes reproducing a specific drawing sequence, $\mathcal{L}_{\text{pixel}}$ only requires that the generated drawing visually matches the image. Like a human, the model should learn to follow one drawing style (a la paint-by-numbers) before learning to draw freely.

==> sections/old/related.tex <==
% !TEX root = ../main.tex
\vspace{-0.1in}
\section{Related Work}
\label{sec:related}
\vspace{-0.1in}
In this section we review relevant literature including generating sketch-like images, unsupervised representation learning, unsupervised few-shot classification and sketch-based image retrieval (SBIR).

{\bf Autoregressive drawing models:}
~\citet{gravesrnn} use an LSTM to directly output the pen coordinates to imitate handwriting sequences. SketchRNN~\citep{ha2017sketchrnn} builds on this by applying it to general sketches beyond characters. \citet{learn2sketchcycle, aisketcher, sketchformer} all extend SketchRNN through architectural improvements.~\citet{chen2017pix2seq} change inputs to be pixel images. This  and the previous 3 works consider multi-class sketching, but none handle more than 20 classes. Autoregressive models also generate images directly in the pixel domain. DRAW~\citep{draw} uses recurrent attention to plot pixels; ~\citet{oneshotgen} extends this to one-shot generation and PixelCNN~\citep{pixelcnn} generates image pixels sequentially. 

{\bf Image processing methods \& GANs:} Other works produce sketch-like images based on style transfer or low-level image processing techniques. Classic methods are based on edge detection and image segmentation~\citep{ucm,hed}.~\citet{fcr} use a CNN to directly produce sketch-like pixels for face images. Photo-sketch and pix2pix~\citep{photosketch,pix2pix} propose a conditional GAN to generate images across different style domains. Image processing based methods do not acquire high-level image understanding, as all the operations are in terms of low-level filtering; none of the GAN sketching methods are designed to mimic human drawings on open domain natural images.

{\bf Unsupervised representation learning:}
In the sketch image domain, our method is similar to the large category of generative models which learn unsupervised representations by the principle of analysis-by-synthesis. Work by \citet{handwrittenmotor} operates in a sketch domain and learns to draw by synthesizing an interpretable motor program. Bayesian Program Learning~\citep{Lake2015bpl} draws through exact inference of common strokes but learning and inference are computationally challenging. As such, a variety of deep generative models aim to perform approximate Bayesian inference by using an encoder structure that directly predicts the embedding, e.g., deep autoencoders~\citep{sae}, Helmholtz Machine~\citep{dayan1995helmholtz}, variational autoencoder (VAE)~\citep{vae}, BiGAN~\citep{donahue2016bigan}, etc. Our method is also related to the literature of self-supervised representation learning~\citep{context,jigsaw,rotation,colorization}, as sketch strokes are part of the input data itself. In few-shot learning~\citep{vinyals2016matching,snell2017prototypical,finn2017maml}, recent work has explored unsupervised meta-training. CACTUs, AAL and UMTRA \citep{hsu2018cactus, antoniou2019assume, khodadadeh2019umtra} all operate by generating pseudo-labels for training.

{\bf Sketch-based image retrieval (SBIR): }
In SBIR, a model is provided a sketch-drawing and retrieves a photo of the same class. The area is split into fine-grained (FG-SBIR)~\citep{sketchshoe, Sangkloy2016sketchy, sketchlessformore} and a zero-shot setting (ZS-SBIR)~\citep{cyclesbir, stackedsbir, doodletosketch}. FG-SBIR considers minute details while ZS-SBIR learns high-level cross-domain semantics and a joint latent space to perform retrieval.

==> sections/old/tab_alpha_values.tex <==
% \begin{table}[t]
% \vspace{-0.1in}
% \centering
% \caption{Effect of pixel loss coefficient $\alpha$ on Omniglot few-shot classification}
% \label{tab:alpha_values}
% \resizebox{0.45\textwidth}{!}{
% \begin{tabular}{cc}
% \toprule
% $\alpha_\text{max}$ & 20-way 1-shot Acc.     \\
% \midrule
% 0.00                & 87.17 $\pm$ 0.36 \\
% 0.25                & 87.82 $\pm$ 0.36 \\
% 0.50                & \textbf{91.39} $\pm$ 0.31 \\
% 0.75                & 90.59 $\pm$ 0.32 \\ 
% 0.95                & 89.77 $\pm$ 0.32 \\
% \endrule
% \end{tabular}}
% \vspace{-0.1in}
% \end{table}

==> sections/old/tab_architecture_comparison.tex <==
\begin{table*}[H]
    \centering
    \caption{Model comparisons between generative autoregressive models that produce pixel or vector sketch drawings.}
    \resizebox{0.98\textwidth}{!}{
    % model - dataset - # classes - encoder - decoder - loss 
    \begin{tabular}{@{}llllll@{}}
\toprule
\multicolumn{6}{c}{\textbf{Autoregressive sketching models}} \\ 
\midrule
\textbf{Model} & \textbf{Dataset} & \textbf{\# classes} & \textbf{Encoder} & \textbf{Decoder} & Loss function \\
\midrule
Handwriting Sequence \cite{gravesrnn} & IAM-OnDB \cite{iamondb} & 1 & RNN & Mixture Density RNN & $\mathcal{L}_\text{stroke}$ \\
DRAW \cite{draw} & SVHN\cite{svhn}, MNIST \cite{mnist} & 10 & RNN & RNN & $\mathcal{L}_\text{pixel} + \mathcal{L}_\text{KL}$ \\
Sketch-RNN \cite{ha2017sketchrnn} & Quickdraw \cite{jongejan2016quickdraw} & 1 & Bi-directional RNN & Mixture Density RNN & $\mathcal{L}_\text{pen} + \mathcal{L}_\text{stroke} + \mathcal{L}_\text{KL}$ \\
Sketch-pix2seq \cite{chen2017pix2seq} & Quickdraw \cite{jongejan2016quickdraw} & 3, 6 & simple CNN & Mixture Density RNN & $\mathcal{L}_\text{pen} + \mathcal{L}_\text{stroke}$ \\
AI-Sketcher \cite{aisketcher} & \makecell[l]{Quickdraw \cite{jongejan2016quickdraw}, \\ FaceX \cite{aisketcher}} & 5, 10, 15, 20 & \makecell[l]{Bi-directional RNN \\+ CNN Autoencoder} & Mixture Density RNN & $\mathcal{L}_\text{pen} + \mathcal{L}_\text{stroke} + \mathcal{L}_\text{KL}$ \\
deep\_p2s \cite{learn2sketchcycle} & \makecell[l]{Quickdraw \cite{jongejan2016quickdraw}, \\ ShoesV2 \cite{sketchshoe}, ChairV2} & 1 & Bi-directional RNN, CNN & CNN, Mixture Density RNN & \makecell[l]{$\mathcal{L}_\text{pen} + \mathcal{L}_\text{stroke} + \mathcal{L}_\text{l2}$ \\ $+ \mathcal{L}_\text{KL} + \mathcal{L}_\text{shortcut}$} \\
\midrule
\model{} \textit{(ours)} & Quickdraw \cite{jongejan2016quickdraw} & 300 & ResNet12 \cite{oreshkin2018tadam} & Mixture Density RNN & $\mathcal{L}_\text{pen} + \mathcal{L}_\text{stroke} + \mathcal{L}_\text{pixel}$ \\
\bottomrule
    \end{tabular}}
    \label{tab:sketch_arch_comparison}
\end{table*}

==> sections/old/tab_miniimagenet_main.tex <==
% !TEX root = ../main.tex
\begin{table}[t]
    \vspace{\topbreak{}}
    \caption{Few-shot classification results on mini-ImageNet}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{@{}lllllll@{}}
\toprule
%  few-shot classification
\multicolumn{3}{c}{\textbf{mini-ImageNet}}& \multicolumn{4}{c}{\textbf{(way, shot)}}         \\ \midrule
\textbf{Algorithm}       & \textbf{Backbone} & \textbf{Train Data} & \multicolumn{1}{c}{\textbf{(5,1)}} & \multicolumn{1}{c}{\textbf{(5,5)}} & \multicolumn{1}{c}{\textbf{(5,20)}} & \multicolumn{1}{c}{\textbf{(5,50)}}        \\ \midrule
Training from Scratch   \citep{hsu2018cactus} & N/A & mini-ImageNet       & 27.59 $\pm$ 0.59 & 38.48 $\pm$ 0.66 & 51.53 $\pm$ 0.72 & 59.63 $\pm$ 0.74  \\ \midrule
% k-NN               \citep{hsu2018cactus} & N/A & mini-ImageNet       & 28.90 $\pm$ 1.25 & 42.25 $\pm$ 0.67 & 56.44 $\pm$ 0.43 & 63.90 $\pm$ 0.38  \\
% Linear Classifier  \citep{hsu2018cactus} & N/A & mini-ImageNet       & 29.44 $\pm$ 1.22 & 39.79 $\pm$ 0.64 & 56.19 $\pm$ 0.43 & 65.28 $\pm$ 0.33  \\
% MLP + Dropout      \citep{hsu2018cactus} & N/A & mini-ImageNet       & 29.03 $\pm$ 0.61 & 39.67 $\pm$ 0.69 & 52.71 $\pm$ 0.62 & 60.95 $\pm$ 0.63  \\
% Cluster Matching         \citep{hsu2018cactus} & N/A & mini-ImageNet       & 22.20 $\pm$ 0.50 & 23.50 $\pm$ 0.52 & 24.97 $\pm$ 0.54 & 26.87 $\pm$ 0.55  \\
CACTUs-MAML              \citep{hsu2018cactus} & Conv4 & mini-ImageNet       & 39.90 $\pm$ 0.74 & 53.97 $\pm$ 0.70 & 63.84 $\pm$ 0.70 & 69.64 $\pm$ 0.63  \\
CACTUs-ProtoNet          \citep{hsu2018cactus} & Conv4 & mini-ImageNet       & 39.18 $\pm$ 0.71 & 53.36 $\pm$ 0.70 & 61.54 $\pm$ 0.68 & 63.55 $\pm$ 0.64  \\
AAL-ProtoNet       \citep{antoniou2019assume} & Conv4 & mini-ImageNet       & 37.67 $\pm$ 0.39 & 40.29 $\pm$ 0.68 &\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-} \\
AAL-MAML           \citep{antoniou2019assume} & Conv4 & mini-ImageNet       & 34.57 $\pm$ 0.74 & 49.18 $\pm$ 0.47 &\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-} \\
UMTRA             \citep{khodadadeh2019umtra} & Conv4 & mini-ImageNet       & 39.93   & 50.73            & 61.11            & 67.15             \\
Random CNN                                   & Conv4 & N/A       & 26.85 $\pm$ 0.31 & 33.37 $\pm$ 0.32 & 38.51 $\pm$ 0.28 & 41.41 $\pm$ 0.28  \\ 
Conv-VAE                                     & Conv4 & mini-ImageNet       & 23.30 $\pm$ 0.21 & 26.22 $\pm$ 0.20 & 29.93 $\pm$ 0.21 & 32.57 $\pm$ 0.20  \\
Conv-VAE                                     & Conv4 & Sketchy       & 23.27 $\pm$ 0.18 & 26.28 $\pm$ 0.19 & 30.41 $\pm$ 0.19 & 33.97 $\pm$ 0.19  \\ 
Random CNN                                   & ResNet12 & N/A                & 28.59 $\pm$ 0.34 & 35.91 $\pm$ 0.34 & 41.31 $\pm$ 0.33 & 44.07 $\pm$ 0.31  \\ 
Conv-VAE                                     & ResNet12 & mini-ImageNet      & 23.82 $\pm$ 0.23 & 28.16 $\pm$ 0.25 & 33.64 $\pm$ 0.27 & 37.81 $\pm$ 0.27  \\
Conv-VAE                                     & ResNet12 & Sketchy            & 24.61 $\pm$ 0.23 & 28.85 $\pm$ 0.23 & 35.72 $\pm$ 0.27 & 40.44 $\pm$ 0.28  \\ \midrule
% \model{}-avg \textit{(ours)}               & Conv4 & Sketchy*                & 37.01  & 51.49  & 61.41  & 65.75  \\
\model{} \textit{(ours)}              & Conv4 & Sketchy*                & 38.61 $\pm$ 0.42 & 53.82 $\pm$ 0.41 & 63.34 $\pm$ 0.35 & 67.22 $\pm$ 0.32 \\
% \model{}-avg \textit{(ours)}               & ResNet12 & Sketchy*             & 38.55  & 54.39  & 65.14  & 69.70  \\
\model{} \textit{(ours)}              & ResNet12 & Sketchy*             & \textbf{40.39} $\pm$ 0.44 & \textbf{57.15} $\pm$ 0.38 & \textbf{67.60} $\pm$ 0.33 & \textbf{71.99} $\pm$ 0.3 \\\midrule
MAML \textit{(supervised)} \citep{finn2017maml}                 & Conv4 & mini-ImageNet       & 46.81 $\pm$ 0.77 & 62.13 $\pm$ 0.72 & 71.03 $\pm$ 0.69 & 75.54 $\pm$ 0.62  \\
ProtoNet \textit{(supervised)} \citep{snell2017prototypical}    & Conv4 & mini-ImageNet       & 46.56 $\pm$ 0.76 & 62.29 $\pm$ 0.71 & 70.05 $\pm$ 0.65 & 72.04 $\pm$ 0.60  \\ \bottomrule
    \end{tabular}
    \begin{tablenotes}\footnotesize
    \item[*] Stroke data used for training
    \end{tablenotes}
    \end{threeparttable}}
    \label{tab:mini-imagenet_results}
    \vspace{-0.18in}
\end{table}

==> sections/old/tab_omniglot_main.tex <==
% !TEX root = ../main.tex
\begin{table}[t]
    \vspace{\topbreak{}}
    \caption{Few-shot classification results on Omniglot}
    \centering
    \resizebox{0.99\textwidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{@{}lllllll@{}}
\toprule
 %few-shot classification
\multicolumn{3}{c}{\textbf{Omniglot}}     & \multicolumn{4}{c}{\textbf{(way, shot)}}         \\ \midrule
\textbf{Algorithm}        & \textbf{Encoder} & \textbf{Train Data} & \multicolumn{1}{c}{\textbf{(5,1)}} & \multicolumn{1}{c}{\textbf{(5,5)}} & \multicolumn{1}{c}{\textbf{(20,1)}} & \multicolumn{1}{c}{\textbf{(20,5)}}        \\ \midrule
Training from Scratch    \citep{hsu2018cactus} & N/A & Omniglot            & 52.50 $\pm$ 0.84 & 74.78 $\pm$ 0.69 & 24.91 $\pm$ 0.33 & 47.62 $\pm$ 0.44  \\ \midrule
% k-NN                     \citep{hsu2018cactus} & N/A & Omniglot            & 57.46 $\pm$ 1.35 & 81.16 $\pm$ 0.57 & 39.73 $\pm$ 0.38 & 66.38 $\pm$ 0.36  \\
% Linear Classifier        \citep{hsu2018cactus} & N/A & Omniglot            & 61.08 $\pm$ 1.32 & 81.82 $\pm$ 0.58 & 43.20 $\pm$ 0.69 & 66.33 $\pm$ 0.36  \\
% MLP + Dropout            \citep{hsu2018cactus} & N/A & Omniglot            & 51.95 $\pm$ 0.82 & 77.20 $\pm$ 0.65 & 30.65 $\pm$ 0.39 & 58.62 $\pm$ 0.41  \\
% Cluster Matching         \citep{hsu2018cactus} & N/A & Omniglot            & 54.94 $\pm$ 0.85 & 71.09 $\pm$ 0.77 & 32.19 $\pm$ 0.40 & 45.93 $\pm$ 0.40  \\
CACTUs-MAML              \citep{hsu2018cactus} & Conv4 & Omniglot            & 68.84 $\pm$ 0.80 & 87.78 $\pm$ 0.50 & 48.09 $\pm$ 0.41 & 73.36 $\pm$ 0.34  \\
CACTUs-ProtoNet          \citep{hsu2018cactus} & Conv4 & Omniglot            & 68.12 $\pm$ 0.84 & 83.58 $\pm$ 0.61 & 47.75 $\pm$ 0.43 & 66.27 $\pm$ 0.37  \\
AAL-ProtoNet        \citep{antoniou2019assume} & Conv4 & Omniglot            & 84.66 $\pm$ 0.70 & 88.41 $\pm$ 0.27 & 68.79 $\pm$ 1.03 & 74.05 $\pm$ 0.46  \\
AAL-MAML            \citep{antoniou2019assume} & Conv4 & Omniglot            & 88.40 $\pm$ 0.75 & 98.00 $\pm$ 0.32 & 70.20 $\pm$ 0.86 & 88.30 $\pm$ 1.22  \\
UMTRA              \citep{khodadadeh2019umtra} & Conv4 & Omniglot            & 83.80            & 95.43            & 74.25            & 92.12             \\ 
Random CNN                                     & Conv4 & N/A                 & 67.96 $\pm$ 0.44 & 83.85 $\pm$ 0.31 & 44.39 $\pm$ 0.23 & 60.87 $\pm$ 0.22  \\
Conv-VAE                                       & Conv4 & Omniglot            & 77.83 $\pm$ 0.41 & 92.91 $\pm$ 0.19 & 62.59 $\pm$ 0.24 & 84.01 $\pm$ 0.15  \\
Conv-VAE                                       & Conv4 & Quickdraw           & 81.49 $\pm$ 0.39 & 94.09 $\pm$ 0.17 & 66.24 $\pm$ 0.23 & 86.02 $\pm$ 0.14  \\ \midrule
\model{} \textit{(Ours)}               & Conv4 & Omniglot*            & 94.88 $\pm$ 0.22 & 99.01 $\pm$ 0.08 & 86.18 $\pm$ 0.18 & 96.69 $\pm$ 0.07  \\
% \model{}-avg  \textit{(Ours)}               & Conv4 & Quickdraw*           & 96.37            & 99.43            & 90.69            & 98.07 \\ 
\model{} \textit{(Ours)}               & Conv4 & Quickdraw*           & \textbf{96.96} $\pm$ 0.17 & \textbf{99.50} $\pm$ 0.06 & \textbf{91.67} $\pm$ 0.14 & \textbf{98.30} $\pm$ 0.05  \\ \midrule
MAML \textit{(Supervised)} \citep{finn2017maml}                 & Conv4 & Omniglot            & 94.46 $\pm$ 0.35 & 98.83 $\pm$ 0.12 & 84.60 $\pm$ 0.32 & 96.29 $\pm$ 0.13  \\
ProtoNet \textit{(Supervised)} \citep{snell2017prototypical}    & Conv4 & Omniglot            & 98.35 $\pm$ 0.22 & 99.58 $\pm$ 0.09 & 95.31 $\pm$ 0.18 & 98.81 $\pm$ 0.07  \\ \bottomrule
    \end{tabular}
    \begin{tablenotes}\footnotesize
    \item[*] Stroke data used for training
    \end{tablenotes}
    \end{threeparttable}}
    \label{tab:omniglot_results}
    \vspace{-0.18in}
\end{table}

==> sections/old/tab_resnet_score.tex <==
% !TEX root = ../main.tex
\begin{table}[t]
% \vspace{-0.1in}
\begin{minipage}[t]{0.4\textwidth}
    \begin{small}
        \begin{center}
            \caption{Effect of pixel loss coefficient $\alpha$ on Omniglot few-shot classification}
            \label{tab:alpha_values}
            \resizebox{!}{1.3cm}{
            \begin{tabular}{cc}
            \toprule
            $\alpha_\text{max}$ & 20-way 1-shot Acc.     \\
            \midrule
            0.00                & 87.17 $\pm$ 0.36 \\
            0.25                & 87.82 $\pm$ 0.36 \\
            0.50                & \textbf{91.39} $\pm$ 0.31 \\
            0.75                & 90.59 $\pm$ 0.32 \\ 
            0.95                & 89.77 $\pm$ 0.32 \\
            \bottomrule
            \end{tabular}}
        \end{center}
    \end{small}
\end{minipage}
\hfill
\begin{minipage}[t]{0.55\textwidth}
    \begin{small}
        \begin{center}
        \caption{ResNet-101 45-way classification score on 1-shot generated sketches of seen and unseen classes.}
        \label{tab:generative_scores}
            \resizebox{!}{1.0cm}{
            \begin{tabular}{ccc}
            \toprule
            \textbf{Generation Method}  & \textbf{Seen}  & \textbf{Unseen} \\ \midrule
            Original Data         & 97.66         & 96.09         \\ \midrule
            Conv-VAE              & 76.28 $\pm$ 0.93 & 75.07 $\pm$ 0.84 \\
            \drawmodel{}       & {\bf 81.44} $\pm$ 0.95 & {\bf 77.94} $\pm$ 1.07 \\ \bottomrule
            \end{tabular}}
        \end{center}
    \end{small}
\end{minipage}
\vspace{-0.15in}
\end{table}


==> sections/old/unused/additional_experiments.tex <==
\section{Additional Experiments}
%Was going to explore the over train time and over pixel_weight sweep here. Definitely won't fit now.

==> sections/old/unused/experiments.tex <==
% !TEX root = ../main.tex
\section{Experiments}

\subsection{Setup}

\subsection{Unsupervised few-shot classification}
\begin{table}[h]
  \caption{\centering Unsupervised few-shot classification results. Accuracy in \% of $N$-way $K$-shot learning methods on Omniglot and mini-ImageNet datasets.}
  \label{table:unsupervised few-shot}
  \centering
  \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{llllllllll}
\hline
                          &                     & \multicolumn{4}{c}{\textbf{Omniglot}}                                                                         & \multicolumn{4}{c}{\textbf{mini-ImageNet}}                                                    \\ \hline
\textbf{Algorithm (N, K)} & \textbf{Clustering} & \textbf{(5, 1)}       & \textbf{(5, 5)}       & \textbf{(20, 1)}      & \multicolumn{1}{l|}{\textbf{(20, 5)}} & \textbf{(5, 1)}       & \textbf{(5, 5)}       & \textbf{(5, 20)}      & \textbf{(5, 50)}      \\ \hline
Training from scratch     & N/A                 & 52.50                 & 74.78                 & 24.91                 & \multicolumn{1}{l|}{46.62}            & 27.59                 & 38.48                 & 51.53                 & 59.63                 \\ \hline
k - Nearest Neighbours    & BiGAN               & 49.55                 & 68.06                 & 27.37                 & \multicolumn{1}{l|}{46.70}            & 25.56                 & 31.10                 & 37.31                 & 43.60                 \\
linear classifier         & BiGAN               & 48.28                 & 68.72                 & 27.80                 & \multicolumn{1}{l|}{45.82}            & 27.08                 & 33.91                 & 44.00                 & 50.41                 \\
MLP with dropout          & BiGAN               & 40.54                 & 62.56                 & 19.92                 & \multicolumn{1}{l|}{40.71}            & 22.91                 & 29.06                 & 40.06                 & 48.36                 \\
cluster matching          & BiGAN               & 43.96                 & 58.62                 & 21.54                 & \multicolumn{1}{l|}{31.06}            & 24.63                 & 29.49                 & 33.89                 & 36.13                 \\
CACTUs-MAML               & BiGAN               & 58.18                 & 78.66                 & 35.56                 & \multicolumn{1}{l|}{58.62}            & 36.24                 & 51.28                 & 61.33                 & 66.91                 \\
CACTUs-ProtoNets          & BiGAN               & 54.74                 & 71.69                 & 33.40                 & \multicolumn{1}{l|}{50.62}            & 36.62                 & 50.16                 & 59.56                 & 63.27                 \\
k - Nearest Neighbours    & ACAI / DC           & 57.46                 & 81.16                 & 39.73                 & \multicolumn{1}{l|}{66.38}            & 28.90                 & 42.25                 & 56.44                 & 63.90                 \\
linear classifier         & ACAI / DC           & 61.08                 & 81.82                 & 43.20                 & \multicolumn{1}{l|}{66.33}            & 29.44                 & 39.79                 & 56.19                 & 65.28                 \\
MLP with dropout          & ACAI / DC           & 51.95                 & 77.20                 & 30.65                 & \multicolumn{1}{l|}{58.62}            & 29.03                 & 39.67                 & 52.71                 & 60.95                 \\
cluster matching          & ACAI / DC           & 54.94                 & 71.09                 & 32.19                 & \multicolumn{1}{l|}{45.93}            & 22.20                 & 23.50                 & 24.97                 & 26.87                 \\
CACTUs-MAML               & ACAI / DC           & 68.84                 & 87.78                 & 48.09                 & \multicolumn{1}{l|}{73.36}            & 39.90                 & 53.97                 & 63.84                 & 69.64                 \\
CACTUs-ProtoNets          & ACAI / DC           & 68.12                 & 83.58                 & 47.75                 & \multicolumn{1}{l|}{66.27}            & 39.18                 & 53.36                 & 61.54                 & 63.55                 \\
UMTRA                     & N/A                 & 83.80                 & 95.43                 & 74.25                 & \multicolumn{1}{l|}{92.12}            & 39.93                 & 50.73                 & 61.11                 & 67.15                 \\ \midrule
% ULDA-Protonets            & N/A                 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-}                & \textbf{40.63}        & 55.41                 & 63.16                 & 65.20                 \\
% ULDA-MetaOptNet           & N/A                 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-}                & \textbf{40.71}        & 54.49                 & 63.58                 & 67.65                 \\ \hline
UMTRA (Transfer)          & N/A                 & 87.81                 & \multicolumn{1}{c}{-} & 73.43                 & \multicolumn{1}{c|}{-}                & 34.33                 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
SketchEmbedding (ours)    & N/A                 & \textbf{96.29}        & \textbf{99.54}        & \textbf{91.19}        & \multicolumn{1}{l|}{\textbf{98.55}}   & 39.24                 & \textbf{55.44}        & \textbf{66.11}        & \textbf{70.66}        \\ \hline
MAML (Supervised)         & N/A                 & 94.46                 & 98.83                 & 84.60                 & \multicolumn{1}{l|}{96.29}            & 46.81                 & 62.13                 & 71.03                 & 75.54                 \\
ProtoNets (Supervised)    & N/A                 & 98.35                 & 99.58                 & 95.31                 & \multicolumn{1}{l|}{98.81}            & 46.56                 & 62.29                 & 70.05                 & 72.04                
    \end{tabular}}
\end{table}
\paragraph{Omniglot} 
Def Include.
Unsupervised method.
Supervised.
Fuse embedding?

\paragraph{mini-ImageNet}
Def Include.
Unsupervised, semi-supervisde, supervised(optional)
Fuse embedding(easy for vae, not so easy for acai/bigan/deepcluste,umtra,uldar)?
implement the strongest model, use it as a comparison point

\subsection{Example generation}

\paragraph{Image Generation Scores: ResNet score, Protonet score}
resnet for quickdraw
protonet for omniglot

\paragraph{Guess Drawing Game}
[Figure: how this is set up.]
in-domain component w/ qd/omni
pretty important, might work
primarily for [quickdraw/omniglot]

[if we have time....
Sketchy drawing guessing
few-shot domain adaptation
train a protonet on generated sketches,
have it classify the ground truth sketches]

\paragraph{Visualization of few-shot generation}https://www.overleaf.com/project/5e9625e0acbace000101ba3e
Comparison with baselines. A figure comparison.

\subsection{Least priority: Classification and generation over training}
if we have extra extra tiem.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}[h]
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

==> sections/old/unused/model.tex <==
% !TEX root = ../main.tex
\section{Model}

Here we define the model components for visual concept learning through drawing imitation and the downstream applications of our learned embedding function. A high-level schematic of our experimental setup can be seen in Figure \ref{fig:1_hlsetup}. During train time we learn drawing imitation (A) informed by a drawing loss $\mathcal{L}_\text{draw}$. At test time we evaluate the informativeness of our latent embedding and generative capacity in tasks (B) and (C).

\begin{figure}
    \centering
    \includegraphics[width=0.98\textwidth]{primaryfigs/panel_with_gen_and_zArtboard 1.png}
    \caption[]{\centering Sketch Embedding experimental setup \\
    Note that while the model adds a stroke at teach decoder timestep, the input at that timestep is the concatenation between $z$ and the previous stroke, not the drawing thus far.}
    \label{fig:1_hlsetup}
\end{figure}

\subsection{Drawing imitation}
We perform natural image to sketch domain transfer and drawing imitation through an image-to-sequence, encoder-decoder model similar to \cite{chen2017pix2seq, ha2017sketchrnn}. We make a novel contribution with the addition of a novel pixel-based loss that relaxes the ordering of a sequence of strokes.

\paragraph{Data} Training data for drawing imitation consists of examples $(\bm{x}^{(i)}, \bm{y}^{(i)})$ where $\bm{x}^{(i)} \in \mathbb{R}^{W\times H \times C}$ is an input pixel image and our label $\bm{y}^{(i)} \in \mathbb{R}^{N_s \times 5}$ is our drawing consisting of sequences of strokes. We preserve no notion of class data during training time and combine all examples across train classes to compose our training data.

\paragraph{Architecture}  
Our model is an encoder-decoder architecture where we use a CNN encoder to embed the input pixel image and then decode it as a sketch drawing. We use the recurrent, autoregressive, mixture density network from \cite{ha2017sketchrnn} as described in our background section. While we borrow the idea of a CNN encoder from Sketch-pix2seq\cite{chen2017pix2seq}, we swap their encoder for the ResNet \cite{He2016resnet} based encoder used in the TADAM architecture \cite{oreshkin2018tadam}. 

Our latent space $z \in \mathbb{R}^{256}$ is a random multivariate Gaussian distribution parameterized by our encoder. We do not enforce any prior on this latent space through the use of any KL loss objective.

\paragraph{Training and objectives} We train the model for drawing imitation in an end-to-end fashion by optimizing 3 different quantities; a pen loss $\mathcal{L}_{\text{pen}}$, a mixture density network (MDN) $\mathcal{L}_{\text{MDN}}$ loss as well as our novel pixel loss $\mathcal{L}_{\text{pixel}}$.

The mutually exclusive pen-state predictions are optimized as a simple 3-way classification through a softmax cross-entropy as the pen loss $\mathcal{L}_{\text{pen}}$.
\begin{align}
    \mathcal{L}_{\text{pen}} &= -\frac{1}{N_s}\sum_{n=1}^{N_s}\sum_{m=1}^3 p_{m, n}\text{log}(q_{m,n})
\end{align}
The MDN loss maximizes the log-likelihood of the offsets of every stroke $(\Delta x, \Delta y)$ in our label drawing $\bm{y}$ given the parameter outputs at that timestep. The term in the inner sum is the probability from Equation \ref{equation:offset_probability}.
\begin{align}
    \mathcal{L}_{\text{MDN}} = -\frac{1}{N_s}\sum_{i=1}^{N_s}\text{log}\big(\sum_{j=1}^{M}\Pi_{j,i} \mathcal{N}(\Delta x_{i}, \Delta y_{i} | \mu_{x,j,i}, \mu_{y,j,i}, \sigma_{x,j,i}, \sigma_{y,j,i}, \rho_{xy,j,i})\big) 
\end{align}
For the pixel loss, we apply a differentiable rasterization function $f_{\text{raster}}$ to our strokes $\mathbf{y}$ and a sequence sampled from our decoder outputs $\mathbf{S}$ to produce two pixel images. Then we apply a Gaussian blurring $g$ and then compute the binary cross-entropy loss. Details on our rasterization function can be found in Appendix \ref{appendix:rasterization}.
\begin{align}
    I &= g(f_{\text{raster}}(\mathbf{y})) \\
    \hat{I} &= g(f_{\text{raster}}(\mathbf{S})) \\
    \mathcal{L}_{\text{pixel}} &= -\frac{1}{WH}\sum_{i=1}^W \sum_{j=1}^H I_{ij} \text{log}(\hat{I}_{ij})
\end{align}

Throughout training we increase a weighting parameter $\alpha$ from $0$ to prioritize $L_{\text{raster}}$ over $L_{\text{pen}}$ as training continues. We find that $\alpha$ is an important hyperparameter that impacts both the learned embedding space and the generation quality of our model.
\begin{align}
    \mathcal{L}_{\text{draw}} = \mathcal{L}_{\text{pen}} + \alpha \mathcal{L}_{\text{pixel}} + (1-\alpha)\mathcal{L}_{\text{MDN}}
\end{align}
While the same sketch can be drawn in many ways, $L_{\text{pen}}$ reproduces a specific drawing sequence while $L_{\text{pixel}}$ only requires that the end drawing visually representative. Like a human, the model should learn to draw one way before learning to draw freely.

\subsection{Few-shot classification}
We evaluate our model in the setting of unsupervised few-shot image classification. Not only are class labels not present during training time, our drawing model is trained on entirely different data distributions as the few-shot benchmarks we look to compare to. As such, the only labels present in a $N$-way $K$-shot few-shot classification episode are the $N \times K$ labels present in the support set.

First we treat our CNN encoder as a deterministic embedding function $f_\text{embed}$ by taking only the mean value of the latent space $z$. We apply this embedding function to every image input in our few-shot task. We then train a simple linear classifier on the embedded support set and use that to classify the embedded query set. 

\subsection{Example Generation}
Like most encoder-decoder and latent embedding models we are able to repeatedly generate instances of a given class through a single input image. Our model has two sources of stochasticity, first in the random normal distribution of our embedding space and secondly in the sampling of points from the mixture of bivariate Gaussians at each decoding timestep. Unlike most generative models that produce variations through different placements of pixel intensities, samples from our model vary in offsets and pen states of each stroke.
